Pinpoint Counterfactuals: Reducing social bias in foundation models via localized counterfactual generation

Foundation models trained on web-scraped datasets propagate societal biases to downstream tasks. While counterfactual generation enables bias analysis, existing methods introduce artifacts by modifying contextual elements like clothing and background. We present a localized counterfactual generation method that preserves image context by constraining counterfactual modifications to specific attribute-relevant regions through automated masking and guided inpainting. When applied to the Conceptual Captions dataset for creating gender counterfactuals, our method results in higher visual and semantic fidelity than state-of-the-art alternatives, while maintaining the performance of models trained using only real data on non-human-centric tasks. Models fine-tuned with our counterfactuals demonstrate measurable bias reduction across multiple metrics, including a decrease in gender classification disparity and balanced person preference scores, while preserving ImageNet zero-shot performance. The results establish a framework for creating balanced datasets that enable both accurate bias profiling and effective mitigation.

==> sec/7_discussion.tex <==
\section{Discussion}

A key advantage of the proposed approach is that it preserves the real distributions of concepts not explicitly expressing the protected attributes of people. In other words, it adds diversity to the distributions of protected attributes but does not alter any other information. Thus, models trained on the data generated with this method do not demonstrate a drop in performance on generic recognition problems, such as ImageNet zero-shot classification (see Figure \ref{fig_in1k}).

Interestingly, as was discussed in Section~\ref{sec_realsim_results} and shown in Table~\ref{table_image_realism}, many state-of-the-art image realism metrics fail to correctly assess the realism of synthetic images, returning lower scores for the actual real data. This could potentially be explained by the fact that the models that are used in these metrics are over-optimized to the local image features, such as smoothness and color intensity, failing to capture high-level semantic information that serves as a better cue for realism.

Furthermore, the experiments presented in Section \ref{sec_results_finetuning} may indicate that CLIP learns to associate gender with context and clothing rather than the actual physiological cues, and switching the gender in the images may harm the learned representations and negatively affect the downstream performance. For example, 
the finetuning setups c4 and c5 in Table \ref{table_finetuning} contain real images of women and inpainted images of men (starting from the images of women and men, respectively). As can be seen from the table, when the inpainted images of men originate from a different gender (switching the gender), we observe a drop in performance on ImageNet, gender classification and the recognition for the class \textit{``dancer''}. Similarly, the setup c9 that switches both genders leads to significant degradation of the model's gender recognition capacity. %\textcolor{red}{I think it is going to be more clear when the results for c7 and c10 are ready - for now it is just a hypothesis I have. Another \textbf{hypothesis} is that the problem is the switching of men because they appear in less diverse clothes than women (i.e., a woman in "neutral" or "manly" clothes is more likely than a man in a dress), and the switching may mess up the learned representations.}

Finally, the experiments outlined in Table \ref{table_image_retrieval}, show that the proposed inpainting approach does not seem to affect the performance on other protected attributes. We conjecture that this is the result of conditioning on the source image's content that leads to the replication of the person's attribute in the inpainted image.
